Solving the swing-up and balance task for the Acrobot and Pendubot with SAC

We present a solution of the swing-up and balance task for the pendubot and acrobot for the participation in the AI Olympics competition at IJCAI 2023. Our solution is based on the Soft Actor Crtic (SAC) reinforcement learning (RL) algorithm for training a policy for the swing-up and entering the region of attraction of a linear quadratic regulator(LQR) controller for stabilizing the double pendulum at the top position. Our controller achieves competitive scores in performance and robustness for both, pendubot and acrobot, problem scenarios.

==> Makefile <==
DOCUMENT = main
DOCUMENT_TEX=$(DOCUMENT).tex

all: pdf

pdf:
	pdflatex $(DOCUMENT_TEX)
	@if grep -qe citation $(DOCUMENT).aux; then\
		bibtex $(DOCUMENT);\
	fi
	pdflatex $(DOCUMENT_TEX)
	@if grep -qe istfilename $(DOCUMENT).aux; then\
		makeglossaries $(DOCUMENT);\
	fi
	pdflatex $(DOCUMENT_TEX)
	pdflatex $(DOCUMENT_TEX)


clean:
	rm -f *.aux *.bbl *.blg *.comments *.lof *.lot *.log *.out *.pdf *.toc *.tcp *.versions *.glg *.glo *.gls *.ist *.log

